Radiation of relativistic electrons created in tunnel ionization of atomic gases by laser beams of extreme intensity

We consider tunnel ionization of atomic argon in a femtosecond laser pulse of intensity $10^{21}-10^{22}{\rm W/cm}^2$ aiming to investigate the relativistic dynamics and radiation of photoelectrons released from their parent ions inside the laser focus. Radiation of such electrons accelerated along the laser field propagation direction appears to have moderate power but can be considerably enhanced by a collision with a relatively weak counter-propagating laser pulse. Using the theory of laser-induced tunneling in atoms and ions and that of nonlinear Thomson scattering, we demonstrate that angular distributions and spectra of emitted photons can serve as a probe of the peak intensity in the focus. The angular distribution of emitted radiation in the plane of polarization and propagation of the ionizing laser beam appears narrow and peaked around an intensity-dependent angle, making this ionization setup a source of collimated XUV radiation.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
\usepackage{float}
\usepackage{dcolumn}
\usepackage{caption}
